Empirical Mass and Radius Relations for Main-sequence Stars from Detached Eclipsing Binaries

Detached eclipsing binaries have long served as fundamental calibrators for stellar models because they provide precise measurements of stellar masses and radii. Given a sample of detached eclipsing binaries, we can derive empirical relations between spectroscopic parameters (effective temperatures, surface gravities and abundances) and stellar masses and radii. We use a sample of 605 stars (330 with metallicities) in detached eclipsing binaries to update and refine these empirical models for main-sequence stars. An eight-term polynomial model reproduces the radii and masses of the eclipsing binary calibrators with an RMS scatter of $\sigma_{\log R} = 0.0161$ dex (3.8%) and $\sigma_{\log M} = 0.0322$ dex (7.7%), respectively. Most of this scatter is explained by the parameter uncertainties - the estimated intrinsic scatters in the radius and mass are only $\sigma_{\rm int}=0.0085$ and $0.017$ dex (2.0% and 4.0%). The predicted mass and radius of the Sun are $(1.028\pm0.004)\ M_\odot$ and $(1.014\pm0.002)\ R_\odot$. A 14-term model, while formally preferred, explains little more of the intrinsic scatter. We additionally provide the equivalent relations in terms of the mean stellar density instead of the surface gravity for use with exoplanet host stars. If we compare the 8-term model to MIST and PARSEC model stars with closely matched spectroscopic parameters, we find systematic differences. For example, the radii of hot (cool) stars are systematically over- (under-)estimated in both models by several percent.

==> ANC/01_eb_sample_macros.tex <==
% generated by notebooks/01_eb_sample.ipynb; do not edit by hand
\newcommand{\ndebcat}{312}
\newcommand{\ndebcatcomponents}{595}
\newcommand{\neb}{325}
\newcommand{\nebcomponents}{621}
\newcommand{\tefferrfill}{140}
\newcommand{\tefferrfloor}{50}
\newcommand{\ntefferrfloor}{40}
\newcommand{\nloggmismatch}{24}

